On Avoiding Power-Seeking by Artificial Intelligence

We do not know how to align a very intelligent AI agent's behavior with human interests. I investigate whether -- absent a full solution to this AI alignment problem -- we can build smart AI agents which have limited impact on the world, and which do not autonomously seek power. In this thesis, I introduce the attainable utility preservation (AUP) method. I demonstrate that AUP produces conservative, option-preserving behavior within toy gridworlds and within complex environments based off of Conway's Game of Life. I formalize the problem of side effect avoidance, which provides a way to quantify the side effects an agent had on the world. I also give a formal definition of power-seeking in the context of AI agents and show that optimal policies tend to seek power. In particular, most reward functions have optimal policies which avoid deactivation. This is a problem if we want to deactivate or correct an intelligent agent after we have deployed it. My theorems suggest that since most agent goals conflict with ours, the agent would very probably resist correction. I extend these theorems to show that power-seeking incentives occur not just for optimal decision-makers, but under a wide range of decision-making procedures.

==> macros.tex <==
% TikZ styles
\RequirePackage{pgf}
\RequirePackage{tikz}
\RequirePackage{qtree}
\usetikzlibrary{arrows,automata,positioning,arrows.meta,bending,calc}
\def\opacity{.1}
\def\smallradius{.25cm}
\def\graphColor{red} % Color to use for involution, etc
\tikzstyle{blue}=[% Define these with arguments?
    shape = circle,
    draw = blue,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = blue
]
\tikzstyle{gray}=[
    shape = circle,
    draw = gray,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = gray
]
\tikzstyle{red}=[
    shape = circle,
    draw = red,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = red
]
\tikzstyle{green}=[
    shape = circle,
    draw = green,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = green
]
\tikzstyle{purple}=[
    shape = circle,
    draw = purple,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = purple
]
\tikzstyle{black}=[
    shape = circle,
    draw = black,
    fill = white,
    minimum size = .1cm,
    font= \small,
    text = black
]
\tikzstyle{hide}=[
    shape = circle,
    draw = white,
    fill opacity = .9,
    fill = white,
    minimum size = .5cm,
    text = black
]
\tikzstyle{hideArr}=[
    shape = circle,
    draw = black,
    opacity = \opacity,
    fill = black,
    text = black
]

\renewcommand{\star}{\textrm{\ding{72}}}
\renewcommand{\triangleright}{{\vartriangleright}}
\renewcommand{\triangleleft}{{\vartriangleleft}}


% Generic math notation
\renewcommand{\abs}[1]{\left|#1\right|}
\newcommand*{\prn}[1]{\left(#1\right)}
\newcommand*{\brx}[1]{\left[#1\right]}
\renewcommand{\set}[1]{\left\{#1\right\}}
\newcommand*{\defeq}{\coloneqq} % definitions
\newcommand*{\eqdef}{\eqqcolon} % definitions
\newcommand*{\x}{\mathbf{x}} % generic row vector
\newcommand*{\av}{\mathbf{a}}
\newcommand*{\bv}{\mathbf{b}}
\newcommand*{\cv}{\mathbf{c}}
\newcommand*{\independent}{\perp \!\!\!\! \perp} % Conditional independence relation
\newcommand*{\dimGen}{d}

% Add arg in parentheses if input is not empty
\newcommand*{\prnNotEmpty}[1]{\ifthenelse{\isempty{#1}}
    {}
    {\prn{#1}}
}

% Misc math
\newcommand*{\reals}{\mathbb{R}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\newcommand*{\unitvec}[1][s]{\mathbf{e}_{#1}}
\newcommand*{\permute}[1][\phi]{\mathbf{P}_{#1}} % permutation matrix
\newcommand*{\upsc}[1]{\text{\upshape\textsc{#1}}}

% Book-keeping for the table of definitions
\newcommand*{\rowskip}{\\[1pt]}

% Acronyms
\newcommand*{\mdp}[1][m]{{\textsc{#1dp}}}
\newcommand*{\rsd}[1][r]{{\textsc{#1sd}}}
\newcommand*{\rl}[1][r]{{\textsc{#1l}}}
\NewDocumentCommand{\iid}{}{\textsc{iid}}

% Standard RL notation
\newcommand*{\St}{\mathcal{S}}
\newcommand*{\A}{\mathcal{A}}
\newcommand*{\rf}{\mathbf{r}} % column-vector reward function
\newcommand*{\uf}{\mathbf{u}} % column-vector utility function
\newcommand*{\rewardSpace}{\reals^{\St}} % reward function space
\newcommand*{\rewardVS}{\reals^{\abs{\St}}} % reward vector space
\newcommand*{\genVS}{\reals^{\dimGen}}
\newcommand*{\boundedRewards}{[0,1]^{\abs{\St}}} % reward vector space
\newcommand{\stateEnd}{$1$-cycle}
\newcommand*{\terminal}{terminal}

% Value functions
\NewDocumentCommand{\Vf}{O{*}O{R}m}{V^{#1}_{#2} \prn{#3}}
\NewDocumentCommand{\VfNoResize}{O{*}O{R}m}{V^{#1}_{#2} (#3)}
\NewDocumentCommand{\VfNorm}{O{*}O{R}m}{\Vf[#1][#2,\,\text{norm}]{#3}}

\NewDocumentCommand{\OptVf}{O{R}m}{\Vf[*][#1]{#2}}
\newcommand*{\OptVfNorm}[2][R]{\VfNorm[*][#1]{#2}}

\newcommand*{\Vfmin}[2][R]{\Vf[\min][#1]{#2}}
\newcommand*{\VfminNorm}[2][R]{\Vfmin[#1,\,\text{norm}]{#2}}

\newcommand*{\OptQfNorm}[2][R]{Q^*_{#1,\,\text{norm}}\prn{#2}}

% Optimal policy set function
\NewDocumentCommand{\piSet}{O{}O{R,\gamma}}{\Pi^{#1}\prn{#2}}
\newcommand*{\optPi}{\piSet[*]}
\newcommand*{\greedy}[1][R]{\piSet[\text{greedy}][#1]}
\newcommand*{\average}[1][R]{\piSet[\text{avg}][#1]}

% Optimal policy set decomposition
\newcommand*{\POpt}{\mathcal{P}^\text{opt}}
\newcommand*{\polOrderSim}[1][\Pi']{\sim^{#1}}
\newcommand*{\polOrderStrict}[1][\Pi']{\succ^{#1}}  % ordering over state lotteries
\newcommand*{\polActions}[1][s]{\A^{\Pi'}_{#1}}

% Topology
\DeclareMathOperator{\interior}{Int}
\DeclareMathOperator{\bd}{bd}

% Reachability
\newcommand*{\reach}[2][]{\upsc{Reach}_{#1}\prn{#2}}
\newcommand*{\children}[1][s]{Ch\prn{#1}}
\newcommand*{\sureChildren}[1][s]{Ch_\text{sure}\prn{#1}}
\newcommand*{\childDists}[1][s]{{T(#1)}}
\newcommand*{\childDistsNd}[1][s]{T_\text{\upshape\text{nd}}\prn{#1}}
\newcommand*{\bottleneck}[4][s]{#1\to #2\overset{#3}{\to}#4}

% Bottleneck proof shorthand
\newcommand*{\rest}{\text{rest}}
\newcommand*{\reachT}{\text{reach}}
\newcommand*{\Fbrest}{F^b_\rest}
\newcommand*{\FbrestA}[1][a_1]{F^b_{\rest,#1}}
\newcommand*{\frest}{\f_\rest}
\newcommand*{\onerest}{\indic{\rest}}
\newcommand*{\onereach}{\indic{\reachT}}
\newcommand*{\fai}[1][a_i]{\f_{#1}}
\newcommand*{\Fbai}[1][a_i]{F^b_{#1}}

% Distributions
\newcommand*{\Dist}{X} % State reward distribution
\newcommand*{\D}{\mathcal{D}} % Joint reward distribution
\DeclareMathOperator{\optSupp}{supp}
\NewDocumentCommand{\supp}{O{\D}}{\optSupp(#1)}
\newcommand*{\opt}[1][\f(\gamma)\geq\F(s,\gamma)]{\optSupp\prn{#1}}
\NewDocumentCommand{\geqMost}{O{}O{\DSetAny}}{\geq_{\text{\upshape {most}}\ifthenelse{\isempty{#2}}{}{\text{\upshape: }#2}}^{#1}}
\NewDocumentCommand{\leqMost}{O{}O{\DSetAny}}{\leq_{\text{\upshape {most}}\ifthenelse{\isempty{#2}}{}{\text{\upshape: }#2}}^{#1}}
\newcommand*{\distSet}{\mathfrak{D}}

% Custom distributions
\NewDocumentCommand{\Diid}{O{\Dist}}{\D_{#1\text{-}\iid}}
\newcommand*{\DSetiid}{\distSet_{\iid}}
\newcommand*{\DSetBCiid}{\distSet_{\textsc{c/b/}\iid}}
\newcommand*{\Dany}{\D_{\text{any}}}
\newcommand*{\DSetAny}{\distSet_\text{any}}
\newcommand*{\Dbd}{\D_{\text{bound}}}
\newcommand*{\DSetBd}{\distSet_\text{bound}}
\newcommand*{\Dcont}{\D_\text{cont}}
\newcommand*{\DSetCont}{\distSet_\text{cont}}
\newcommand*{\Dt}[1][]{\D_\text{#1}} % auxiliary reward function distribution

% Power
\NewDocumentCommand{\vavg}{O{s,\gamma}O{\Dbd}}{\OptVf[#2]{#1}}
\NewDocumentCommand{\vavgNoResize}{O{s,\gamma}O{\Dbd}}{V^*_{#2}(#1)}
\NewDocumentCommand{\pwrNoDist}{}{\upsc{Power}} % upshape ensures that math doesn't slant the smallcaps
\NewDocumentCommand{\pwr}{O{}O{\Dbd}}{\upsc{Power}_{#2} \prnNotEmpty{#1}}
\NewDocumentCommand{\pwrNoResize}{O{}O{\Dbd}}{\upsc{Power}_{#2} (#1)}
\newcommand*{\unifPower}[1][s]{\upsc{UnifPower}(#1,\gamma)}

\newcommand*{\pwrStateOrder}[1][{s,\gamma}]{\geq^{#1}_{\pwr\text{-seek}}}
\newcommand*{\pwrPreorder}[1][{\St,\gamma}]{\succeq^{#1}_{\pwr\text{-seek}}}

% Probability
\DeclareMathOperator*{\Prb}{\mathbb{P}}
\newcommand*{\prob}[2][]{\Prb_{#1}\prn{#2}}
\NewDocumentCommand{\optprob}{O{\D}O{}m}{\noexpandarg\exploregroups\Prb\IfSubStr{\sim}{#1}{}{\nolimits}_{#1}^{#2}\prn{#3}}
\NewDocumentCommand{\avgprob}{O{\D}m}{\optprob[#1]{#2, \text{\upshape average}}}
\NewDocumentCommand{\greedyprob}{O{\D}m}{\optprob[#1]{#2, \text{\upshape greedy}}}

\newcommand*{\quantDist}{P}

\DeclareMathOperator*{\opE}{\mathbb{E}}
\newcommand*{\E}[2]{\opE_{#1}\brx{#2}} % expectation
\newcommand*{\EX}{\opE\brx{\Dist}}
\NewDocumentCommand{\Edraws}{O{\Dist}m}{\opE\brx{\max \text{ of } #2 \text{ draws from } #1}}
\NewDocumentCommand{\dF}{O{\rf}O{F}}{\dif #2(#1)}

% State visit distributions
\newcommand*{\f}{\mathbf{f}} % visit distribution
\newcommand*{\fpi}[2][\pi]{\f^{
\ifthenelse{\isempty{#1}}{}{#1} % Policy
\ifthenelse{\NOT\isempty{#1} \AND \NOT\isempty{#2}}{,}{} % Insert comma if both arguments
\ifthenelse{\isempty{#2}}{}{#2}}} % State

\DeclareMathOperator{\Fop}{\mathcal{F}}
\NewDocumentCommand{\F}{O{}}{\Fop\prnNotEmpty{#1}}
\newcommand*{\FRestrictAction}[3][s]{\F(#1 \mid \pi(#2)=#3)}
\newcommand*{\FRestrictRSD}[2][s]{\F(#1 \mid {\rsd} \in #2)}
\newcommand*{\FRestrictChild}[2][s]{\F(#1 \mid {\textsc{child distribution}} \in #2)}

\newcommand*{\ND}[1]{\upsc{ND}\prn{#1}}
\NewDocumentCommand{\phelper}{mO{\D'}}{p_{#2}\prn{#1}}
\DeclareMathOperator{\Fndop}{\mathcal{F}_{nd}} % non-dominated visit distributions
\NewDocumentCommand{\Fnd}{O{}}{\Fndop\prnNotEmpty{#1}}
\newcommand*{\FndRestrictAction}[2]{\Fnd(s \mid \pi(#1)=#2)}
\newcommand*{\FRestrict}[1]{\F(s \mid \pi^*, #1)}
\newcommand*{\FndRestrict}[1]{\Fnd(s \mid \pi^*, #1)}  % Multi-state Fnd restriction
\DeclareMathOperator{\Fnonstat}{\F^\text{HD}} % Non-stationary visit distribution functions
\newcommand*{\NormF}[1]{\upsc{Norm}\prn{#1}}

% Recurrent state distributions
\newcommand*{\dbf}{\mathbf{d}} % recurrent state distribution
\newcommand*{\RSD}[1][s]{\upsc{RSD}\prn{#1}}
\newcommand*{\RSDnd}[1][s]{\upsc{RSD}{\text{\upshape\textsubscript{nd}}}\prn{#1}}
\newcommand*{\RSDndNoResize}[1][s]{\upsc{RSD}{\text{\upshape\textsubscript{nd}}}(#1)}

% Column vector
\newcount\colveccount
\newcommand*\colvec[1]{
        \global\colveccount#1
        \protect\begin{pmatrix}
        \colvecnext
}
\def\colvecnext#1{
        #1
        \global\advance\colveccount-1
        \ifnum\colveccount>0
                \\
                \expandafter\colvecnext
        \else
                \protect\end{pmatrix}
        \fi
}

% Suboptimal policies
\newcommand*{\pol}[1][R,\gamma]{\text{pol}\prnNotEmpty{#1}}
\NewDocumentCommand{\pwrPol}{O{\pol[]}O{\Dbd}m}{\pwrNoDist^{#1}_{#2} \prnNotEmpty{#3}}

% Norms
\newcommand*{\lone}[1]{\left \lVert#1\right \rVert_1}
\newcommand*{\linfty}[1]{\left \lVert#1\right \rVert_\infty}

% Fractions
\newcommand*{\geom}[1][1]{\frac{#1}{1-\gamma}}
\newcommand*{\half}{\frac{1}{2}}

\newcommand*{\indic}[1]{\mathbbm{1}_{#1}} % indicator function
\newcommand*{\inv}{^{-1}}

% Permutation groups
\newcommand*{\mdpPermGroup}{S_{\abs{\St}}}
\newcommand*{\genSym}{S_{\dimGen}}
\NewDocumentCommand{\orbi}{O{\Dbd}O{\abs{\St}}}{S_{#2}\cdot #1}
\newcommand*{\symmFnd}{S_{\Fnd(s)}}

% Colors
\definecolor{blue}{rgb}{.25,.45,.75}
\definecolor{purple}{rgb}{.4667,.1529,.2118}
\definecolor{green}{rgb}{.294,.624,.294}
\definecolor{red}{rgb}{.75,.25,.25}
\definecolor{Crimson}{rgb}{.65,0,0}
\definecolor{DGreen}{rgb}{0,0.624,0.428}

\newcommand{\cmark}{{\color{DGreen}\ding{51}}}
\newcommand{\xmark}{{\color{Crimson}\ding{55}}}

\newcommand*{\col}[2]{{\color{#1}#2}}

\newcommand*{\unfinished}{\col{red}{\textbf{ (Unfinished)}}} % Mark unfinished work

% Theorem environment styles
\newtheorem{thm}{Theorem}[chapter]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{cor-no-num}{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{conj}{Conjecture}
\newtheorem{conjSec}[thm]{Conjecture} % section-titled conjectures
\newtheorem*{remark}{Remark}
\newtheorem*{question}{Question}
\newtheorem{questionSec}[thm]{Question}  % Group conjectures by section
\newtheorem*{thm*}{Theorem} % Unlabelled xr repeats (restatable doesn't work across files)
\newtheorem{reaction}{Reaction}
\newtheorem{response}{Counterargument}

% Attainable utility distance
\newcommand*{\dauTemplate}[4][\D]{d_{#1}^{#3}\ifthenelse{\isempty{#2}}
    {}% if no state dists given
    {\prn{#2 \mid #4}}}
\newcommand*{\dau}[2][\D]{\dauTemplate[#1]{#2}{\textsc{au}}{\gamma}}
\newcommand*{\dauNorm}[3][\D]{\dauTemplate[#1]{#2}{\textsc{au},\text{norm}}{#3}}
\newcommand*{\dtv}[1]{\mathrm{TV}\prnNotEmpty{#1}} % total variation distance
\newcommand*{\wasserstein}[1]{W_1\prnNotEmpty{#1}} % Wasserstein 1-distance

% Regret
\newcommand*{\pregret}[1][]{\upsc{PropRegret}\prnNotEmpty{#1}}
\newcommand*{\piSwitch}[2][\pi^*_R]{\pi_\text{switch}(#2,#1,t)}

% POMDP
\newcommand*{\assistGame}{\mathcal{M}}
\newcommand*{\geomDist}[1][p]{G(#1)}
\newcommand*{\initialDist}{\Prb_\St}
\newcommand*{\hNoop}{a_\text{no-op}^H}
\newcommand*{\pomdp}{\textsc{pomdp}}
\newcommand*{\assistant}{\mathbf{A}}
\newcommand*{\human}{\mathbf{H}}
\newcommand*{\initialState}{s_0}
\newcommand*{\pwrdefault}[1][s]{\pwr[#1,\gamma]}

% AUP terminology
\newcommand*{\R}[1][]{\mathcal{R}_\text{#1}} % reward function set notation
\newcommand*{\aup}{\textsc{aup}}
\newcommand*{\dsag}{\textsc{dsag}}
\newcommand*{\rAUP}{R_\aup}
\newcommand*{\rAUPAssist}{\rAUP^\assistGame}
\newcommand*{\gamAUP}{\gamma_\aup}
\newcommand*{\timeDist}{\mathcal{T}}
\newcommand*{\baseline}{\pi^\varnothing}
\newcommand*{\ravg}{\bar{R}}
\newcommand*{\valSwitch}[2][\pi]{V^{\piSwitch{#1}}_{R, \,\text{norm}}\prn{#2}} % Nest default?
\newcommand*{\rVOI}[1][s,\gamma]{\upsc{VOI}_\D(#1)}
\newcommand*{\rAssist}{R^\assistGame}
\newcommand*{\Options}{\texttt{Options}}
\newcommand*{\Damage}{\texttt{Damage}}

% Ground-truth objective distributions
\newcommand*{\Dtrue}{\D_\text{true}}
\newcommand*{\Dinv}{\D_\text{true-inv}}

% Featurization macros
\newcommand*{\feat}{\mathrm{feat}}
\newcommand*{\featMat}{\mathbf{F}}
\newcommand*{\nfeat}{n_f}
\newcommand*{\featVS}{\reals^{\nfeat}}

% appendix.tex macros
\newcommand*{\retarget}{\Theta}
\newcommand*{\rtparam}{\theta}

% Main illustration macros
\ifluatex
\newcommand*{\start}{\text{\emoji{house}}}
\newcommand*{\startGraph}{\text{\emoji{house}}}
\newcommand*{\sink}{\text{\emoji{video-game}}}
\newcommand*{\topleft}{\text{\emoji{evergreen-tree}}}
\newcommand*{\farleft}{\text{\emoji{palm-tree}}}
\newcommand*{\closeleft}{\text{\emoji{sunflower}}}
\newcommand*{\topright}{\text{\emoji{star}}}
\newcommand*{\farright}{\text{\emoji{sun}}}
\newcommand*{\closeright}{\text{\emoji{crescent-moon}}}
\else
\newcommand*{\start}{\star}
\newcommand*{\startGraph}{\small\bigstar}
\newcommand*{\sink}{\varnothing}
\newcommand*{\topleft}{\ell_{\nwarrow}}
\newcommand*{\farleft}{\ell_{\swarrow}}
\newcommand*{\closeleft}{\ell_{\triangleleft}}
\newcommand*{\topright}{r_{\nearrow}}
\newcommand*{\farright}{r_{\searrow}}
\newcommand*{\closeright}{r_\triangleright}
\fi

\newcommand*{\leftA}{\texttt{left}}
\newcommand*{\rightA}{\texttt{right}}

% Tikz helper
\def\centerarc[#1](#2)(#3)(#4:#5:#6){ \draw[#1] (#2)++(#3) arc (#4:#5:#6); }
\NewDocumentCommand{\arcHelp}{O{0pt}O{0pt}O{.35cm}O{->}mm}{ % O{x offset} O{y offset} O{arc radius} O{arrow settings} m{cardinal direction setting} m{base node}

\ifthenelse{\equal{#5}{N}}{\centerarc[#4](#6.east)(#1,#2)(-50:240:#3)}{}
\ifthenelse{\equal{#5}{NE}}{\centerarc[#4](#6.east)(-1pt++#1,.5pt++#2)(-95:200:#3)}{}
\ifthenelse{\equal{#5}{E}}{\centerarc[#4](#6.east)(#1,-5pt++#2)(-130:145:#3)}{}
\ifthenelse{\equal{#5}{SE}}{\centerarc[#4](#6.east)(-9pt++#1,-7.5pt++#2)(-180:110:#3)}{}
\ifthenelse{\equal{#5}{S}}{\centerarc[#4](#6.south)(7pt++#1,-1pt++#2)(40:-235:#3)}{}
\ifthenelse{\equal{#5}{SW}}{\centerarc[#4](#6.west)(8.5pt++#1,-8pt++#2)(0:-290:#3)}{}
\ifthenelse{\equal{#5}{W}}{\centerarc[#4](#6.west)(#1,-6pt++#2)(-35:-325:#3)}{}
\ifthenelse{\equal{#5}{NW}}{\centerarc[#4](#6.west)(-1pt++#1,3.5pt++#2)(250:-15:#3)}{}
}

%% SafeLife sprites

\newcommand{\inlinesprite}[2]{
  \begingroup\normalfont\hspace{-0.5em}
  \raisebox{-.1\height}{\includegraphics[height=0.65em, clip, trim={#1}]{chapters/complex/sprites/sprites-#2.pdf}}
  \hspace{-0.22em}\endgroup
}
\DeclareRobustCommand {\agentsprite}[1][gray]    {\inlinesprite{2cm 4cm 2cm 0cm}{#1}}
\DeclareRobustCommand {\lifesprite}[1][gray]     {\inlinesprite{0cm 3cm 4cm 1cm}{#1}}
\DeclareRobustCommand {\hardlifesprite}[1][gray]  {\inlinesprite{1cm 3cm 3cm 1cm}{#1}}
\DeclareRobustCommand {\weedsprite}[1][gray]      {\inlinesprite{2cm 3cm 2cm 1cm}{#1}}
\DeclareRobustCommand {\plantsprite}[1][gray]    {\inlinesprite{3cm 3cm 1cm 1cm}{#1}}
\DeclareRobustCommand {\treesprite}[1][gray]     {\inlinesprite{3cm 1cm 1cm 3cm}{#1}}
\DeclareRobustCommand {\icesprite}[1][gray]      {\inlinesprite{0.02cm 2.02cm 4cm 2cm}{#1}}
\DeclareRobustCommand {\fountainsprite}[1][gray] {\inlinesprite{1cm 2cm 3cm 2cm}{#1}}
\DeclareRobustCommand {\wallsprite}[1][gray]     {\inlinesprite{2cm 2cm 2cm 2cm}{#1}}
\DeclareRobustCommand {\cratesprite}[1][gray]     {\inlinesprite{3cm 2cm 1cm 2cm}{#1}}
\DeclareRobustCommand {\predsprite}[1][gray]     {\inlinesprite{4cm 2cm 0cm 2cm}{#1}}
\DeclareRobustCommand {\spawnsprite}[1][gray]    {\inlinesprite{1cm 1cm 3cm 3cm}{#1}}
\DeclareRobustCommand {\exitsprite}[1][gray]     {\inlinesprite{2cm 1cm 2cm 3cm}{#1}}

% SafeLife conditions
\newcommand*{\naive}{\texttt{Naive}}
\newcommand*{\aupTT}{\texttt{AUP}}
\newcommand*{\aupp}{\texttt{AUP}$_\text{proj}$}

\newcommand*{\dqn}{\texttt{DQN}}
\newcommand*{\ppo}{\texttt{PPO}}

% Author info
\newcommand{\authorinfo}[2]{\ifbool{Dissertate}{}{%
    #1\par
    #2
}}

% my abstract
\newenvironment{myabstract}{\section*{Abstract}}{}

\definecolor{options}{rgb}{.651, .459, .318}
\definecolor{agent}{rgb}{.3, .3, .999}
\definecolor{goal}{rgb}{.012, .753, .235}
\definecolor{off-switch}{rgb}{.65, 0, 0}
\definecolor{living}{rgb}{.863, .455, .714}
\definecolor{other}{rgb}{.961, .502, .145}


% Add chapter in lists of for dissertate
% theorems
% definitions
% conjectures (conjSec,question,questionSec)
\newbool{definitions}
\newbool{theorems}
\newbool{conjectures}
\newcommand{\AddLoeChapter}[1]{\ifbool{Dissertate}{\addtocontents{loe}{\protect\LoeChapter{#1}{\thechapter}{\thischaptertitle}}}{}}
\newcommand{\LoeChapter}[3]{\ifbool{#1}{\vspace{\baselineskip}\parbox[t]{1.45em}{\textsc{#2}}\parbox[t]{\linewidth-2.45em}{\RaggedRight\textsc{#3}}\\[3pt]}{}}

% Dialogue
\newcommand{\refer}[1]{{\normalfont\textsc{#1}}}
\newcommand{\direct}[1]{[\textit{#1}]}
\def\speak#1{\item[{\normalfont\textsc{\lowercase{#1}}:}]}%
\newenvironment{dialogue}{%
    \begin{description}
    }{\end{description}}

% Power-seeking/power-nuances appendix
\newcommand*{\sne}{s_3}
\newcommand*{\sn}{s_2}
\newcommand*{\startApp}{\col{blue}{s_1}}

% Quantitative paper
% Orbits
\newcommand*{\orbInside}[1][\rtparam]{\mathrm{Orbit}|_{\retarget}\prn{#1}}
\newcommand*{\orbInsideCond}[2][\rtparam]{\mathrm{Orbit}|_{\retarget,#2}\prn{#1}}

% Montezuma's revenge
\newcommand*{\jump}{\texttt{jump}}
\newcommand*{\initMR}{s_0}
\newcommand*{\initMRObs}{o_0}
\newcommand*{\mr}{\textsc{mr}}
\newcommand*{\observe}{\mathcal{O}} % Observations
\newcommand*{\featFn}{\textrm{feat}} % featurization

\newcommand*{\invleave}{I_{\text{leave}}}
\newcommand*{\invstay}{I_{\text{stay}}}

\newcommand*{\decide}{\mathrm{decide}}
\newcommand*{\stay}{O_\text{stay}}
\newcommand*{\leave}{O_\text{leave}}
\newcommand*{\validObs}{O_\text{$T$-reach}}
%\newcommand*{\ppo}{\textsc{ppo}}
\newcommand*{\fstubborn}{f_{\text{stubborn}}}
\newcommand*{\fbandit}{f_{\text{bandit}}}
\newcommand*{\frand}{f_{\text{rand}}}
\newcommand*{\fmax}{f_{\text{max}}}
\newcommand*{\fnumeric}{f_{\text{numerical}}}
\newcommand*{\alg}{\mathrm{Alg}}
\newcommand*{\algprob}[1]{\prob[\substack{\pi\sim \decide(\rtparam),\\ \tau \sim \pi\mid \initMR}]{#1}}
\newcommand*{\Best}[1]{\mathrm{Best}\prn{#1}}
\newcommand*{\y}{\mathbf{y}}
\newcommand*{\fracOpt}[1]{\mathrm{FracOptimal}\prn{#1}}
\newcommand*{\abDomain}{\mathbf{E}}
\newcommand*{\powFinite}{\mathcal{P}^\text{finite}\prn{\genVS}}
\newcommand*{\powGenVs}{\mathcal{P}\prn{\genVS}}
\DeclareMathOperator*{\dom}{dom}
\newcommand*{\isOpt}[2]{\mathrm{Optimal}\prn{#1\mid #2}}
\newcommand*{\isAnti}[2]{\mathrm{AntiOpt}\prn{#1\mid #2}}
\newcommand*{\boltz}[3][T]{\mathrm{Boltzmann}_{#1}\prn{#2\mid #3}}
\newcommand*{\satisfice}[3][t]{\mathrm{Satisfice}_{#1}\prn{#2 \mid #3}}
\newcommand*{\best}[1][k]{\textrm{best-of-}k}
\newcommand{\train}{\textrm{train}}
% Card suits
\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
\newcommand*{\lotA}{{\color{gray}{\spadesuit^{\text{B}}}}}
\newcommand*{\lotB}{{\color{gray}{\varheart^{\text{B}}}}}
\newcommand*{\lotC}{{\color{gray}{\vardiamond^{\text{A}}}}}
\newcommand*{\heart}{\lotB}
\newcommand*{\diamnd}{\lotC}
\newcommand*{\spade}{\lotA}

\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\definecolor{Gray}{gray}{0.85}
\definecolor{LightGray}{gray}{.925}
\newcolumntype{G}{>{\columncolor{Gray}}c}
\newcolumntype{g}{>{\columncolor{LightGray}}c}
\newcolumntype{w}{>{\columncolor{white}}c}
% Header for tables
\newcommand*{\headers}{Utility function $\uf'$ & $\overset{\lotA}{10},\overset{\lotB}{5},\overset{\lotC}{0}$& $\overset{\lotA}{10},\overset{\lotB}{0},\overset{\lotC}{5}$& $\overset{\lotA}{5},\overset{\lotB}{10},\overset{\lotC}{0}$& $\overset{\lotA}{5},\overset{\lotB}{0},\overset{\lotC}{10}$& $\overset{\lotA}{0},\overset{\lotB}{10},\overset{\lotC}{5}$& $\overset{\lotA}{0},\overset{\lotB}{5},\overset{\lotC}{10}$}


% TikZ setting for graphs
\tikzset{mygraph/.style={>=latex,shorten >=1pt,auto,node distance=1.5cm,line width=0.1em}}

% em dash
\newcommand{\kemdash}{\kern0.01pt---\kern0.01pt}
\newcommand{\ai}{\textsc{ai}}

\DeclareMathOperator{\sgn}{sgn}
